The Danger Of Arrogance: Welfare Equilibra As A Solution To Stackelberg Self-Play In Non-Coincidental Games

The increasing prevalence of multi-agent learning systems in society necessitates understanding how to learn effective and safe policies in general-sum multi-agent environments against a variety of opponents, including self-play. General-sum learning is difficult because of non-stationary opponents and misaligned incentives. Our first main contribution is to show that many recent approaches to general-sum learning can be derived as approximations to Stackelberg strategies, which suggests a framework for developing new multi-agent learning algorithms. We then define non-coincidental games as games in which the Stackelberg strategy profile is not a Nash Equilibrium. This notably includes several canonical matrix games and provides a normative theory for why existing algorithms fail in self-play in such games. We address this problem by introducing Welfare Equilibria (WE) as a generalisation of Stackelberg Strategies, which can recover desirable Nash Equilibria even in non-coincidental games. Finally, we introduce Welfare Function Search (WelFuSe) as a practical approach to finding desirable WE against unknown opponents, which finds more mutually desirable solutions in self-play, while preserving performance against naive learning opponents.

==> Images/WE_figures/ElusiveGame_greedy/figure.tex <==
\begin{figure*}
    \centering
    \captionsetup{justification=centering}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/WE_figures/ElusiveGame_greedy/reward_surface_x/output.pdf}
        \caption{Reward surface for $x$}
        \label{fig:fig:ElusiveGame_greedy reward_surface_x}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/WE_figures/ElusiveGame_greedy/reward_surface_y/output.pdf}
        \caption{Reward surface for $y$}
        \label{fig:fig:ElusiveGame_greedy reward_surface_y}
    \end{subfigure}
    \newline
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/WE_figures/ElusiveGame_greedy/y_br/output.pdf}
        \caption{BR for $y$ as a function of $x$}
        \label{fig:fig:ElusiveGame_greedy y_br}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/WE_figures/ElusiveGame_greedy/x_br/output.pdf}
        \caption{BR for $x$ as a function of $y$}
        \label{fig:fig:ElusiveGame_greedy x_br}
    \end{subfigure}
    \newline
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/WE_figures/ElusiveGame_greedy/br_rewards_x/output.pdf}
        \caption{Rewards as a function of $x$}
        \label{fig:fig:ElusiveGame_greedy br_rewards_x}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Images/WE_figures/ElusiveGame_greedy/br_rewards_y/output.pdf}
        \caption{Rewards as a function of $y$}
        \label{fig:fig:ElusiveGame_greedy br_rewards_y}
    \end{subfigure}
    \caption{Stackelberg strategy profile (Greedy WE) for ElusiveGame \\ $x^* = 0.500, y^* = 1.000, R^x = 0.500, R^y = 0.500$}
    \label{fig:ElusiveGame_greedy}
\end{figure*}

